Linearly dispersive bands at the onset of correlations in K$_x$C$_{60}$ films

Molecular crystals are a flexible platform to induce novel electronic phases. Due to the weak forces between molecules, intermolecular distances can be varied over relatively larger ranges than interatomic distances in atomic crystals. On the other hand, the hopping terms are generally small, which results in narrow bands, strong correlations and heavy electrons. Here, by growing K$_x$C$_{60}$ fullerides on hexagonal layered Bi$_2$Se$_3$, we show that upon doping the series undergoes a Mott transition from a molecular insulator to a correlated metal, and an in-gap state evolves into highly dispersive Dirac-like fermions at half filling, where superconductivity occurs. This picture challenges the commonly accepted description of the low energy quasiparticles as appearing from a gradual electron doping of the conduction states, and suggests an intriguing parallel with the more famous family of the cuprate superconductors. More in general, it indicates that molecular crystals offer a viable route to engineer electron-electron interactions.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

END { system('cp', 'output.bbl', 'paper.bbl'); }
